SPIN: An Empirical Evaluation on Sharing Parameters of Isotropic Networks

Recent isotropic networks, such as ConvMixer and vision transformers, have found significant success across visual recognition tasks, matching or outperforming non-isotropic convolutional neural networks (CNNs). Isotropic architectures are particularly well-suited to cross-layer weight sharing, an effective neural network compression technique. In this paper, we perform an empirical evaluation on methods for sharing parameters in isotropic networks (SPIN). We present a framework to formalize major weight sharing design decisions and perform a comprehensive empirical evaluation of this design space. Guided by our experimental results, we propose a weight sharing strategy to generate a family of models with better overall efficiency, in terms of FLOPs and parameters versus accuracy, compared to traditional scaling methods alone, for example compressing ConvMixer by 1.9x while improving accuracy on ImageNet. Finally, we perform a qualitative study to further understand the behavior of weight sharing in isotropic architectures. The code is available at https://github.com/apple/ml-spin.

==> figures_tex/weight_l2.tex <==
\begin{figure}[th!]
    \centering
    \includegraphics[width=\linewidth]{figures/ConvMixer_L2.png}
    \caption{L2 distance of weights across each layer for 3 pre-trained ConvMixer models.}
    \label{fig:weight_l2}
\end{figure}

==> figures_tex/weight_similarity.tex <==
\begin{figure}[th!]
    \centering
    \begin{subfigure}{0.49\linewidth}
        \includegraphics[width=\linewidth]{figures/convmixer_768_32_7_7.png}
        \caption{ConvMixer-768/32}
        \label{subfig:}
    \end{subfigure}
    \begin{subfigure}{0.49\linewidth}
        \includegraphics[width=\linewidth]{figures/convmixer_1536_20_9_7.png}
        \caption{ConvMixer-1536/20}
        \label{subfig:}
    \end{subfigure}
    \caption{L2 distance and cosine similarity of pre-trained weights across each layer for (a) ConvMixer with 32-layer and 768-channel, and (b) ConvMixer with 20-layer and 1536-channel.}
    \label{fig:weight_sim}
\end{figure}


==> tables/sharing_rates.tex <==
\setlength{\tabcolsep}{4pt}
\begin{table}[t!]
    \centering
    \caption{\textbf{ImageNet Top-1 accuracy of Weight Shared ConvMixer (768/32/14/3) under different sharing rates.} The first row is the results of the standard, non-shared version. Note that for sharing rates under 2, a non-uniform distribution is needed. We only study the Middle distribution for this case as Section \ref{layer-similarity} suggests. The details of the layer structure of Middle distribution can be found in Appendix.}
    \label{tab:sharing_rates}
    \resizebox{0.8\columnwidth}{!}{
        \begin{tabular}{cccccc}
        \toprule[1.5pt]
        Sharing & Sharing & Sharing & Params & FLOPs & ImageNet \\
        Distribution & Mapping & Rate & (M) & (G) & Acc (\%) \\
        \midrule[1pt]
        - & - & - & 20.46 & 5.03 & 75.71  \\
        \midrule
        \multirow{6}{*}{Middle} & \multirow{6}{*}{Sequential} & 1.33 & 15.75 & \multirow{6}{*}{5.03} & ? \\
        & & 1.67 & 13.39 & & ? \\
        & & 2 & 11.02 & & 72.84 \\
        & & 4 & 6.3 & & 69.28 \\
        & & 8 & 3.95 & & 64.46 \\
        \midrule
        \multirow{3}{*}{Uniform} & \multirow{3}{*}{Sequential} & 2 & 11.02 & \multirow{3}{*}{5.03} & 73.29 \\
        & & 4 & 6.3 & & 70.11 \\
        & & 8 & 3.95 & & 66.31 \\
        \bottomrule[1.5pt]
        \end{tabular}
    }
\end{table}
\setlength{\tabcolsep}{1.4pt}
